Network Games Induced Prior for Graph Topology Learning

Learning the graph topology of a complex network is challenging due to limited data availability and imprecise data models. A common remedy in existing works is to incorporate priors such as sparsity or modularity which highlight on the structural property of graph topology. We depart from these approaches to develop priors that are directly inspired by complex network dynamics. Focusing on social networks with actions modeled by equilibriums of linear quadratic games, we postulate that the social network topologies are optimized with respect to a social welfare function. Utilizing this prior knowledge, we propose a network games induced regularizer to assist graph learning. We then formulate the graph topology learning problem as a bilevel program. We develop a two-timescale gradient algorithm to tackle the latter. We draw theoretical insights on the optimal graph structure of the bilevel program and show that they agree with the topology in several man-made networks. Empirically, we demonstrate the proposed formulation gives rise to reliable estimate of graph topology.

==> fig/game/auc_pa_game.tex <==
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{groupplot}[group style={group name=myplot,group size=2 by 1}]
\nextgroupplot[%
% width=6.028in,
% height=4.754in,
% at={(1.011in,0.642in)},
width=3cm,
height=4cm,
scale only axis,
xmin=0,
xmax=20,
xlabel style={font=\color{white!15!black}},
xlabel={\LARGE$\lambda$},
ymin=18.3264256348728,
ymax=22,
ylabel style={font=\color{white!15!black}},
ylabel={\LARGE ${\bf 1}^\top {\bm y}_{linear}^\star(\GSO)$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
xtick={0,5,10,15,20}, % Set x-axis ticks
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=3.0pt, mark=o, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
0.01	18.4387468238589\\
1	18.4887752843917\\
5	18.4888815238208\\
10	18.4864256348728\\
15	18.4887381550742\\
20	18.4812179076843\\
};
%\addlegendentry{sig log}

\addplot [color=mycolor2, dashed, line width=3.0pt, mark=x, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
0.01	18.43926361926\\
1	18.5485665336455\\
5	18.8160909280834\\
10	18.8770011425686\\
15	20.0539531653926\\
20	21.2110279115429\\
};
%\addlegendentry{li}

\addplot [color=mycolor4, dashdotted, line width=3.0pt, mark=diamond, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
0.01	18.4393137275574\\
1	18.4921857792905\\
5	18.5035103869766\\
10	18.5273864514901\\
15	18.6312575997398\\
20	18.7341605090496\\
};
%\addlegendentry{Ab}
\hspace{.5cm}
\nextgroupplot[%
width=3cm,
height=4cm,
% width=6.028in,
% height=4.754in,
% at={(1.011in,0.642in)},
scale only axis,
xmin=0,
xmax=20,
xlabel style={font=\color{white!15!black}},
xlabel={\LARGE$\lambda$},
ymin=7.87393270429137,
ymax=8.2,
ylabel style={font=\color{white!15!black}},
ylabel={\LARGE ${\bf 1}^\top {\bm y}_{\log}^\star(\GSO)$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
xtick={0,5,10,15,20}, % Set x-axis ticks
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=3.0pt, mark=o, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
0.01	7.90141130229592\\
1	7.91912076771596\\
5	7.9181838108102\\
10	7.92193270429137\\
15	7.92101247315915\\
20	7.9192065123094\\
};
%\addlegendentry{sig log}

\addplot [color=mycolor3, dotted, line width=3.0pt, mark=square, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
0.01	7.90144082943361\\
1	7.92245234159815\\
5	7.93028399630737\\
10	7.95956807385192\\
15	8.000050634152\\
20	8.1835651611685\\
};
%\addlegendentry{log}

\addplot [color=mycolor4, dashdotted, line width=3.0pt, mark=diamond, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
0.01	7.90154738286892\\
1	7.92093965919876\\
5	7.92268721253453\\
10	7.9389957917396\\
15	7.94759029707184\\
20	7.96390548683164\\
};
%\addlegendentry{Ab}

\end{groupplot}
\end{tikzpicture}%

==> fig/game/pa_game.tex <==
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{groupplot}[group style={group name=myplot,group size=3 by 1}]
\nextgroupplot[%
width=6cm,
height=4cm,
% at={(1.011in,0.642in)},
scale only axis,
xmin=0,
xmax=20,
xlabel style={font=\color{white!15!black}},
xlabel={\LARGE $\lambda$},
ymin=0.5,
ymax=1.05,
ylabel style={font=\color{white!15!black}},
ylabel={\LARGE AUC},
xtick={0,5,10,15,20}, % Set x-axis ticks
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend pos = north west,
legend style={
legend cell align=left, align=left, 
% at={(0.8,1)},
  draw opacity=0.8,
  text opacity=1,draw=white!15!black,font=\large},
% legend pos=north east
]
% \addplot [color=mycolor1,   line width=2.0pt]
%   table[row sep=crcr]{%
% 0.01	0.727860605107988\\
% 1	0.728553904909174\\
% 5	0.726265369844858\\
% 10	0.729596819827015\\
% 15  0.728370235687948\\
% 20	0.731015429319106\\
% };\label{plots:Smooth-GL}
% % \addlegendentry{Smooth-GL}

\addplot [color=mycolor1, loosely dashed, line width=2.0pt]
  table[row sep=crcr]{%
0.01	0.727860605107988\\
20	0.727860605107988\\
};\label{plots:Smooth-GL}

\addplot [color=black, loosely dashed, line width=2.0pt]
  table[row sep=crcr]{%
0.01	0.519312307770735\\
20	0.519312307770735\\
};\label{plots:xiaowen}

\addplot [color=gray, loosely dashed, line width=2.0pt]
  table[row sep=crcr]{%
0.01	0.904474672466822\\
20	0.904474672466822\\
};\label{plots:spec}

\addplot [color=mycolor2, line width=3.0pt, mark=x, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
0.01	0.727938983670071\\
1	0.737841233495897\\
5	0.783294958283064\\
10	0.804155465683359\\
15  0.88901942259002\\
20	0.904237837516358\\
};\label{plots:bi-x}
% \addlegendentry{Bilevel Opt., $f(x) = x$}

\addplot [color=mycolor3, line width=3.0pt, mark=square, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
0.01	0.727880146646502\\
1	0.7307268390287\\
5	0.735877839895326\\
10	0.747787621709799\\
15  0.781776410814118\\
20	0.808675508504819\\
};\label{plots:bi-log}
% \addlegendentry{Bilevel Opt., $f(x) = \log(x+1)$}

\addplot [color=mycolor4, dashdotted, line width=3.0pt, mark=diamond, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
0.01	0.727866127716699\\
1	0.729027681014121\\
5	0.732983767778552\\
10	0.735949361926286\\
15  0.738285017587385\\
20	0.742011546500366\\
};\label{plots:bi-app}
% \addlegendentry{Linear Approx.}


\nextgroupplot[%
% width=6.028in,
% height=4.754in,
% at={(1.011in,0.642in)},
width=6cm,
height=4cm,
scale only axis,
xmin=0,
xmax=20,
xlabel style={font=\color{white!15!black}},
xlabel={\LARGE$\lambda$},
ymin=18.3264256348728,
ymax=22,
ylabel style={font=\color{white!15!black}},
ylabel={\LARGE ${\bf 1}^\top {\bm y}_{linear}^\star(\GSO)$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
xtick={0,5,10,15,20}, % Set x-axis ticks
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1,loosely dashed,   line width=2.0pt]
  table[row sep=crcr]{%
0.01	18.4387468238589\\
20	18.4387468238589\\
};
%\addlegendentry{sig log}


\addplot [color=mycolor2, line width=3.0pt, mark=x, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
0.01	18.43926361926\\
1	18.5485665336455\\
5	18.8160909280834\\
10	18.8770011425686\\
15	20.0539531653926\\
20	21.2110279115429\\
};
%\addlegendentry{li}

\addplot [color=mycolor4, dashdotted, line width=3.0pt, mark=diamond, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
0.01	18.4393137275574\\
1	18.4921857792905\\
5	18.5035103869766\\
10	18.5273864514901\\
15	18.6312575997398\\
20	18.7341605090496\\
};
%\addlegendentry{Ab}
 \hspace{0.5cm}
\coordinate (top) at (rel axis cs:1,0);

\nextgroupplot[%
width=6cm,
height=4cm,
% width=6.028in,
% height=4.754in,
% at={(1.011in,0.642in)},
scale only axis,
xmin=0,
xmax=20,
xlabel style={font=\color{white!15!black}},
xlabel={\LARGE$\lambda$},
ymin=7.87393270429137,
ymax=8.2,
ylabel style={font=\color{white!15!black}},
ylabel={\LARGE ${\bf 1}^\top {\bm y}_{\log}^\star(\GSO)$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
xtick={0,5,10,15,20}, % Set x-axis ticks
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, loosely dashed,  line width=2.0pt]
  table[row sep=crcr]{%
0.01	7.90141130229592\\
20	7.90141130229592\\
};
%\addlegendentry{sig log}

\addplot [color=mycolor3, dotted, line width=3.0pt, mark=square, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
0.01	7.90144082943361\\
1	7.92245234159815\\
5	7.93028399630737\\
10	7.95956807385192\\
15	8.000050634152\\
20	8.1835651611685\\
};
%\addlegendentry{log}

\addplot [color=mycolor4, dashdotted, line width=3.0pt, mark=diamond, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
0.01	7.90154738286892\\
1	7.92093965919876\\
5	7.92268721253453\\
10	7.9389957917396\\
15	7.94759029707184\\
20	7.96390548683164\\
};
%\addlegendentry{Ab}
\hspace{.7cm}
\coordinate (bot) at (rel axis cs:0,0);% coordinate at bottom of the last plot


\end{groupplot}
\path (top|-current bounding box.north)--
      coordinate(legendpos)
      (bot|-current bounding box.north);
\matrix[
    matrix of nodes,
    anchor=south,
    draw,
    inner sep=0.2em,
    draw,
    font = \large,
  ]at([yshift=1.75ex,xshift=-30ex]legendpos)
  {\ref{plots:Smooth-GL}& {\Large Smooth-GL}&[5pt]
  \ref{plots:bi-x}& {\Large Bilevel Opt., $f(x) = x$}&[5pt]
\ref{plots:bi-log}& {\Large Bilevel Opt., $f(x) = \log(x+1)$}&[5pt]
\ref{plots:bi-app}& {\Large Linear Approx.}
\\
};


\end{tikzpicture}%

==> fig/game/welfare_pa_game.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{groupplot}[group style={group name=myplot,group size=1 by 1}]
\nextgroupplot[%
width=7cm,
height=6cm,
% at={(1.011in,0.642in)},
scale only axis,
xmin=0,
xmax=20,
xlabel style={font=\color{white!15!black}},
xlabel={\LARGE $\lambda$},
ymin=0.7,
ymax=0.95,
ylabel style={font=\color{white!15!black}},
ylabel={\LARGE AUC},
xtick={0,5,10,15,20}, % Set x-axis ticks
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend pos = north west,
legend style={
legend cell align=left, align=left, 
% at={(0.8,1)},
  draw opacity=0.8,
  text opacity=1,draw=white!15!black,font=\large},
% legend pos=north east
]
\addplot [color=mycolor1, line width=3.0pt, mark=o, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
0.01	0.727860605107988\\
1	0.728553904909174\\
5	0.726265369844858\\
10	0.729596819827015\\
15  0.728370235687948\\
20	0.731015429319106\\
};
\addlegendentry{Smooth-GL}

\addplot [color=mycolor2, dashed, line width=3.0pt, mark=x, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
0.01	0.727938983670071\\
1	0.737841233495897\\
5	0.783294958283064\\
10	0.804155465683359\\
15  0.88901942259002\\
20	0.904237837516358\\
};
\addlegendentry{Bilevel Opt., $f(x) = x$}

\addplot [color=mycolor3, dotted, line width=3.0pt, mark=square, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
0.01	0.727880146646502\\
1	0.7307268390287\\
5	0.735877839895326\\
10	0.747787621709799\\
15  0.781776410814118\\
20	0.808675508504819\\
};
\addlegendentry{Bilevel Opt., $f(x) = \log(x+1)$}

\addplot [color=mycolor4, dashdotted, line width=3.0pt, mark=diamond, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
0.01	0.727866127716699\\
1	0.729027681014121\\
5	0.732983767778552\\
10	0.735949361926286\\
15  0.738285017587385\\
20	0.742011546500366\\
};
\addlegendentry{Linear Approx.}
\end{groupplot}
\end{tikzpicture}%




